A Unified Approach to Scalar, Vector, and Tensor Slepian Functions on the Sphere and Their Construction by a Commuting Operator

We present a unified approach for constructing Slepian functions - also known as prolate spheroidal wave functions - on the sphere for arbitrary tensor ranks including scalar, vectorial, and rank 2 tensorial Slepian functions, using spin-weighted spherical harmonics. For the special case of spherical cap regions, we derived commuting operators, allowing for a numerically stable and computationally efficient construction of the spin-weighted spherical-harmonic-based Slepian functions. Linear relationships between the spin-weighted and the classical scalar, vectorial, tensorial, and higher-rank spherical harmonics allow the construction of classical spherical-harmonic-based Slepian functions from their spin-weighted counterparts, effectively rendering the construction of spherical-cap Slepian functions for any tensorial rank a computationally fast and numerically stable task.

==> plotSlep.tex <==
\graphicspath{{SlepPlots4/}}

 \subsection[Implementation of Tensor Slepian Functions for the Polar Cap]{Implementation of Tensor Slepian Functions on the\\Polar Cap}\label{plotslep} 

\noindent We implemented the construction of
tensor Slepian functions for polar cap regions from spin-weighted
spherical harmonics following the description in
Section~\ref{tenslep}. The calculation of the Legendre
polynomials, of the associated Legendre functions, of the spherical
harmonics, and of its derivatives are based on the algorithms
of \cite{fenglerdiss}. We present, as an example, tensor Slepian functions for a 
polar cap with radius $40^\circ = \frac{2}{9}\pi \,\mathrm{rad} $ and
bandlimit $L=18$, the same parameters as in \cite{simons} 
for the scalar Slepian functions. All numerical calculations
were carried out using \texttt{MATLAB R2015b}. The 
total number of tensor Slepian functions is $9(L+1)^2-12=3237$.
For our polar cap of opening angle
$40^\circ$, the rounded Shannon number is
$S\approx 379$.
\newline
\newline
Figure~\ref{plot_shannon} shows the resulting sorted
eigenvalues for our example. The Shannon number is
indicated by the abscissa of the red \lq+\rq . Most of the eigenvalues cluster
either around 0 or 1, with a sharp drop-off in-between. The Shannon
number separates the cluster around 1 from the cluster around
0. The largest eigenvalue is
$\lambda_1=0.999999999403780$, while the smallest eigenvalues
are within machine accuracy of $0$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{tensslep_18_2-9pi_shannon_dots}
\caption{Distribution of the sorted eigenvalues of the tensor Slepian
functions with bandlimit $L=18$ for a polar cap with radius
$40^\circ$. Altogether, we have $9(L+1)^2-12=3237$ functions and the
Shannon number is given by $S\approx 379$. The eigenvalue closest to the Shannon number is marked by a red $+$.}
\label{plot_shannon}
\end{figure}

\alon [XXXX Die Shannonzahl beschreibt eine Anzahl Slepian
funktionen, hat aber keinen Eigenwert. Deshalb sollte sie nicht als
ein Punkt, sondern als eine vertikale linie dargestellt werden (am
besten beim tats\"achlichen wert und nicht beim aufgerundeten wert) XXXX] \aloff \kaon [Wie soll nun die Shannon Zahl eingezeichnet werden?]\kaoff
\newline
\newline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent The resulting Slepian functions are, as their
eigenvalues indicate, ordered by their concentration within the region
of interest. Figures~\ref{plotslep_best1}
to~\ref{plotslep_less2} show the pointwise Euclidean
norm of the tensor Slepian functions for a selection of $\alpha$
 between $1$ and $3237$, the dimension of
$\boldsymbol{\mathrm{harm}}_{0,\ldots,18}(\Omega)$.
 The first few 
tensor Slepian functions are
 well concentrated within the polar cap
marked by the red circle (see
Figures~\ref{plotslep_best1} and~\ref{plotslep_best2}). Those
Slepian functions with index close to the Shannon number are
concentrated around the boundary of the polar cap
(see~Figure \ref{plotslep_shannon1}). Finally, the least
concentrated functions are localized within the complementing
region (i.e.~the south-polar cap of opening angle~$140^\circ$). In
general, the least concentrated tensor Slepian functions of the
spherical cap at the North pole defined by $t\in\lbrack b,1\rbrack$
are the best concentrated Slepian functions of the 
south-polar cap defined by $t\in\lbrack -1,-1+b\rbrack$ (see
Figure \ref{plotslep_less2}) and their concentration values are
 $1-\lambda_\alpha$. Even though the functions themselves are not equal, there
are groups of tensor Slepian functions whose pointwise Euclidean norms are identical (as functions on the sphere). This is a consequence of the
same spin-weighted Slepian functions being multiplied by different
unit tensors (see Equation~\ref{SlepTensTypes}).
\newline
\newline
Figure~\ref{plotslep_shannon1} shows the Slepian functions with
indices close to the Shannon number. The bottom row confirms 
that the Shannon number, as expected, is a good estimate for the
indices of the well-concentrated Slepian functions. The tensor
Slepian function whose index is closest to the Shannon
number is concentrated at the boundary of the polar 
cap. About half of these functions' energy is concentrated
outside of the region of interest, as is evident from the bottom row
of Figure~\ref{plotslep_shannon1}, but also from the corresponding
eigenvalues. Michel and Simons therefore suggest 
in \cite{michelsimons} to use a number smaller than the Shannon number
as a better estimate for the number of Slepian functions that are
well concentrated within the region of interest. The functions shown
in the upper row of Figure~\ref{plotslep_shannon1} are still 
concentrated at the boundary of the polar cap but are
more focused on the interior area of the polar cap.
\newline
\newline
 Figure~\ref{plotslep_less2} shows the Slepian functions with the
highest indices and hence the lowest energy concentration within the
target region (and highest energy concentration within the
complementing region). The bottom-right panel of 
Figure~\ref{plotslep_less2} presents the same function, for
index $\alpha=3237$, as the bottom-left panel, but in the Robinson
projection, to highlight that the energy of this Slepian function is
concentrated at the South Pole. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
\begin{minipage}{8.25cm}
\includegraphics[width=8.25cm]{tensslep_18_2-9pi_w1}
\end{minipage}
%
\begin{minipage}{8.25cm}
\includegraphics[width=8.25cm]{tensslep_18_2-9pi_w10}
\end{minipage}
\begin{minipage}{8.25cm}
\includegraphics[width=8.25cm]{tensslep_18_2-9pi_w28}
\end{minipage}
%
\begin{minipage}{8.25cm}
\includegraphics[width=8.25cm]{tensslep_18_2-9pi_w46}
\end{minipage}
 
\caption{Azimuthal equidistant polar projection of the pointwise
Euclidean norm of the best-concentrated tensor Slepian functions for a
polar cap with radius $40^\circ$ and bandlimit $L=18$. The cap is
indicated by a solid red line. The Slepian functions are for indices
$\alpha=1$ (top-left), $\alpha=10$ (top-right), $\alpha=28$
(bottom-left) and $\alpha=46$ (bottom-right).}
\label{plotslep_best1}
 
\end{figure}

\begin{figure}
\begin{minipage}{8.25cm}
\includegraphics[width=8.25cm]{tensslep_18_2-9pi_w55}
\end{minipage}
%
\begin{minipage}{8.25cm}
\includegraphics[width=8.25cm]{tensslep_18_2-9pi_w73}
\end{minipage}
\begin{minipage}{8.25cm}
\includegraphics[width=8.25cm]{tensslep_18_2-9pi_w91}
\end{minipage}
%
\begin{minipage}{8.25cm}
\includegraphics[width=8.25cm]{tensslep_18_2-9pi_w109}
\end{minipage}
 
\caption{Azimuthal equidistant polar projection of the pointwise
Euclidean norm of the best-concentrated tensor Slepian functions for a
polar cap with radius $40^\circ$ and bandlimit $L=18$. The cap is
indicated by a solid red line. The Slepian functions are for indices
$\alpha=55$ (top-left), $\alpha=73$ (top-right), $\alpha=91$
(bottom-left) and $\alpha=109$ (bottom-right).}
\label{plotslep_best2}
 
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
\begin{minipage}{8.25cm}
\includegraphics[width=8.25cm]{tensslep_18_2-9pi_w304}
\end{minipage}
%
\begin{minipage}{8.25cm}
\includegraphics[width=8.25cm]{tensslep_18_2-9pi_w324}
\end{minipage}
\begin{minipage}{8.25cm}
\includegraphics[width=8.25cm]{tensslep_18_2-9pi_w379}
\end{minipage}
%
\begin{minipage}{8.25cm}
\includegraphics[width=8.25cm]{tensslep_18_2-9pi_w391}
\end{minipage}
 
\caption{Azimuthal equidistant polar projection of the pointwise
Euclidean norm of the tensor Slepian functions with index close to the
Shannon number for a polar cap with radius $40^\circ$ and bandlimit
$L=18$. The cap is indicated by a solid red line. The Slepian
functions are for indices $\alpha=304$ (top-left), $\alpha=324$
(top-right), $\alpha=379$ (bottom-left) and $\alpha=391$
(bottom-right). The rounded Shannon number is~$379$.}
\label{plotslep_shannon1}
 
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
\begin{minipage}{8.25cm}
\includegraphics[width=8.25cm]{tensslep_18_2-9pi_w3228}
\end{minipage}
%
\begin{minipage}{8.25cm}
\includegraphics[width=8.25cm]{tensslep_18_2-9pi_w3233}
\end{minipage}
\begin{minipage}{8.25cm}
\includegraphics[width=8.25cm]{tensslep_18_2-9pi_w3237}
\end{minipage}
%
\begin{minipage}{8.25cm}
\includegraphics[width=8.25cm]{tensslep_18_2-9pi_w3237_global}
\end{minipage}
 
\caption{Pointwise Euclidean norm of the least-concentrated tensor Slepian
functions for a polar cap with radius $40^\circ$ and bandlimit
$L=18$. The cap is indicated by a solid red line. The Slepian
functions are for indices $\alpha=3228$ (top-left, azimuthal
equidistant polar projection), $\alpha=3233$ (top-right, azimuthal
equidistant polar projection), and $\alpha=3237$ (bottom left:
azimuthal equidistant polar projection, bottom right: Robinson
projection)}
\label{plotslep_less2}
 
\end{figure}


